Higgs compositeness in $\mathrm{Sp}(2N)$ gauge theories --- The pure gauge model

As a first step in the study of $\mathrm{Sp}(2N)$ composite Higgs models, we obtained a set of novel numerical results for the pure gauge $\mathrm{Sp}(4)$ lattice theory in 3+1 space-time dimensions. Results for the continuum extrapolations of the string tension and the glueball mass spectrum are presented and their values are compared with the same quantities in neighbouring $\mathrm{SU}(N)$ models.

==> contspectrum.tex <==
$ A1^+ $ & $ 3.557(52) $ \\
%$ A1^{+*} $ & $ 6.05(4) $ \\
$ A1^- $ & $ 5.74(19) $ \\
%$ A1^{-*} $ & $ 7.81(8) $ \\
$ A2^+ $ & $ 7.91(17) $ \\
$ A2^- $ & $ 9.42(40) $ \\

